Information geometry of operator scaling

Matrix scaling is a classical problem with a wide range of applications. It is known that the Sinkhorn algorithm for matrix scaling is interpreted as alternating e-projections from the viewpoint of classical information geometry. Recently, a generalization of matrix scaling to completely positive maps called operator scaling has been found to appear in various fields of mathematics and computer science, and the Sinkhorn algorithm has been extended to operator scaling. In this study, the operator Sinkhorn algorithm is studied from the viewpoint of quantum information geometry through the Choi representation of completely positive maps. The operator Sinkhorn algorithm is shown to coincide with alternating e-projections with respect to the symmetric logarithmic derivative metric, which is a Riemannian metric on the space of quantum states relevant to quantum estimation theory. Other types of alternating e-projections algorithms are also provided by using different information geometric structures on the positive definite cone.

==> prelim.tex <==
\section{Preliminaries}~\label{sec:pre}
\subsection{Classical information geometry}
%\subsection{Affine connection, dual connections, and flatness}
We assume basic knowledge of Riemannian geometry (see, e.g., \cite{AmariNagaoka2007}).
Let $(M,g)$ be a smooth Riemannian manifold with a metric tensor $g$. 
Let $\nabla$ be an affine connection.
A coordinate system $(\theta^i)$ is called an \emph{affine coordinate system} for $\nabla$ if the Christoffel symbols of $\nabla$ with respect to $(\theta^i)$ vanish: $\Gamma_{ij}^k = 0$ for all $i,j,k$.
An affine connection $\nabla$ is \emph{flat} if it has an affine coordinate system.
Affine connections $\nabla$ and $\nabla^*$ are \emph{dual} to each other if 
\begin{align*}
    Z g(X, Y) = g(\nabla_Z X, Y) + g(X, \nabla^*_Z, Y)
\end{align*}
for all vector fields $X$, $Y$, and $Z$.
A tuple $(g, \nabla, \nabla^*)$ is called a \emph{dualistic structure} of $M$.
We say that $(M, g, \nabla, \nabla^*)$ is a \emph{dually flat space} if $\nabla$ and $\nabla^*$ are both flat.

A curve $\gamma(t)$ in $M$ is called a \emph{$\nabla$-geodesic} if $\nabla_{\dot\gamma} \dot\gamma = 0$. 
Especially, a $\nabla$-geodesic from $p$ to $q$ is a $\nabla$-geodesic $\gamma(t)$ with $\gamma(0) = p$ and $\gamma(1)=q$.
Let $M'$ be a submanifold of $M$ and $p$ be a point in $M$.
A point of $q$ in $M'$ is a \emph{$\nabla$-projection} of $p$ on $M'$ if any tangent vector in $T_p(M')$ is orthogonal to the $\nabla$-geodesic between $p$ and $q$ at $q$.
For a flat connection $\nabla$, a submanifold $M'$ is said to be \emph{$\nabla$-flat} if $M'$ can be represented as an affine subspace in an affine coordinate system of $\nabla$.

%\subsection{Dually flat spaces and canonical divergence}
A dually flat space $(M,g,\nabla,\nabla^*)$ has beautiful connection to convex analysis.
Let $[\eta_i]$ and $[\theta^i]$ be affine coordinate systems for $\nabla$ and $\nabla^*$, respectively.
Then, there exists a unique strictly convex function $\psi$ such that 
\[
    \eta_i = \frac{\partial \psi }{\partial \theta^i}.
\]
Furtheremore, $\nabla^*$-projection can be characterized by \emph{divergence minimization}. 
More precisely, for a $\nabla$-flat submanifold $M'$ and a point $p \in M$, $q \in M'$ is $\nabla^*$-projection of $p$ if and only if
\[
    q \in \argmin_{q' \in M'} D_\psi(q' \mid\mid p),
\]
where $D_\psi$ is the Bregman divergence
\[
    D(q \mid\mid p) = \psi(q) - \psi(p) + \inprod{\grad\psi(p), q-p}.
\]
Furthermore, it satisfies the \emph{generalized Pythagorean theorem}
\[
    D(q' \mid\mid p) = D(q' \mid\mid q) + D(q \mid\mid p) 
\]
where $p \in M$, $q$ is the $\nabla^*$-projection of $p$ on $M'$, and $q' \in M'$.
%In classical information geometry, the Fisher metric is the only monotone metric (Cencov's theorem).

\subsection{Quantum information geometry}
Here, we briefly summarize several notations of quantum information geometry.

A quantum system is associated with a Hilbert space.
For example, a qubit system is associated with $\mathbb{C}^2$.
We consider finite-dimensional Hilbert space in this study.
A state of a quantum system is described by a density matrix, which is defined as a Hermitian operator $\rho$ that satisfies $\tr \rho=1$ and $\rho\ge 0$.
%The state of a quantum system is described by a density operator.
%We denote the set of all density operators on $\cH$ as $\cS(\cH)$.
%Denote the set of all linear operators on Hilbert space $\cH$ by $\cL(\cH)$ and the set of all positive linear operator by $\cL_+(\cH) \subset \cL(\cH)$.
%For a quantum system with a finite dimensional Hilbert space $\cH$, 
%its quantum state is described by a density operator $\rho$ on $\cH$.
%A Hermitian operator $\rho$ on $\cH$ is a density operator if it satisfies
%\begin{align*}
%\tr \rho=1,\quad \rho\ge 0.
%\end{align*}
%We denote the set of all density operators on $\cH$ as $\cS(\cH)$.
Let us denote by $\caS_{+}$ and $\caS_{++}$ the set of $n\times n$ positive semidefinite and positive definite Hermitian matrices, respectively.
Naturally, we can regard $\caS_{++}$ as a smooth real manifold.

Unlike classical information geometry, monotone metrics are not unique in quantum information geometry.
\cite{Petz1996} showed that each monotone metric is characterized by an operator monotone function.
Each monotone metric induces its own e-connection.
For example, the symmetric logarithmic derivative (SLD) metric is defined as
\[
g_{\rho}^{\mathrm{S}}(X,Y) = \frac{1}{2} \mathrm{tr}\ (L_X^{\mathrm{S}} \rho + \rho L_X^{\mathrm{S}}) L_Y^{\mathrm{S}}, \quad X \rho = \frac{1}{2} (L_X^{\mathrm{S}} \rho + \rho L_X^{\mathrm{S}}).
\]
For a tangent vector $X \in T_\rho(\caS_{++})$ at $\rho \in \caS_{++}$, the \emph{symmetric logarithmic derivative} is the matrix $L_X$ satisfying an Lyapunov equation
\begin{align}\label{eq:SLD}
\rho L_X + L_X\rho = 2X(\rho). 
\end{align}
Note that since $\rho$ is positive definite and $X(\rho)$ is Hermitian, the Lyapunov equation has the unique Hermitian solution.
The \emph{symmetric logarithmic derivative metric (SLD metric)} on $T_\rho(S)$ is defined as 
\begin{align}\label{eq:SLD-metric}
    g(X, Y) = \tr[X(\rho) L_Y].
\end{align}

Let $\nabla$ be the flat connection induced by the Euclidean geometry in $\caS_{++}$ and $\nabla^*$ be its dual connection.
Since $\nabla$ is the flat connection, the geodesic $\gamma$ from $\rho_0$ to $\rho_1$ is given by 
\[
    \gamma(t) = (1-t)\rho_0 + t\rho_1,
\]
which is the standard Euclidean geodesic of $\caS_{++}$.
On the other hand, it is known that the $\nabla^*$-geodesic from $\rho_0$ to $\rho_1$ is given by
\begin{align}\label{eq:SLD-geodesic}
    \gamma(t) = K^t \rho_0 K^t
\end{align}
for $t \in [0,1]$, 
where $K = \rho_1 \# \rho_0^{-1}$ is the matrix geometric mean of $\rho_0^{-1}$ and $\rho_1$.
Adopting the standard terminology of information geometry, we call $\nabla$-geodesic and $\nabla^*$-geodesic by m-geodesic and e-geodesic, respectively.
Furthermore, we call the symmetric logarithmic derivative $L_X$ the e-representation of a tangent vector $X$.

We note that the above dualistic structure $(g, \nabla, \nabla^*)$ is not dually flat in general (see \cite[Chapter~7]{AmariNagaoka2007}). 

\subsection{Useful facts of matrix analysis}
We use tools from matrix analysis in our proof. For the detail, refer to books of Hiai~and~Petz~\cite{HiaiPetz2014}, and Bhatia~\cite{Bhatia2009positive}.

\emph{Partitioned matrices} are matrices with the following block structure:
\begin{align*}
    \begin{bmatrix}
        A_{11} & \cdots & A_{1n} \\
        \vdots & \ddots & \vdots \\
        A_{m1} & \cdots & A_{mn} 
    \end{bmatrix},
\end{align*}
where $A_{ij} \in \C^{m'\times n'}$ for all $i$ and $j$. 
Slightly abusing the notation, we write the set of partitioned matrices by $\C^{m\times n} \otimes \C^{m'\times n'}$.
For matrices $A = (a_{ij}) \in \C^{m\times n}$ and $B=(b_{kl}) \in \C^{m' \times n'}$, the \emph{Kronecker product} is a partitioned matrix defined as
\begin{align*}
    A \otimes B = 
    \begin{bmatrix}
        a_{11} B & \cdots & a_{1n} B \\
        \vdots & \ddots & \vdots \\
        a_{m1} B & \cdots & a_{mn}B 
    \end{bmatrix}
    \in \C^{m\times n}\otimes \C^{m'\times n'}.
\end{align*}
For partitioned matrices with $m=n$ and $m'=n'$, we define \emph{partial traces} as 
\begin{align*}
    \tr_1
    \begin{bmatrix}
        A_{11} & \cdots & A_{1n} \\
        \vdots & \ddots & \vdots \\
        A_{n1} & \cdots & A_{nn} 
    \end{bmatrix} &= \sum_{i=1}^n A_{ii}, \\
    \tr_2
    \begin{bmatrix}
        A_{11} & \cdots & A_{1n} \\
        \vdots & \ddots & \vdots \\
        A_{n1} & \cdots & A_{nn} 
    \end{bmatrix} &= 
    \begin{bmatrix}
        \tr A_{11} & \cdots & \tr A_{1n} \\
        \vdots & \ddots & \vdots \\
        \tr A_{n1} & \cdots & \tr A_{nn} 
    \end{bmatrix}.
\end{align*}

Let $A \in \C^{n\times n}$ be a Hermitian matrix (i.e., $A = A^\dagger$) with the spectral decomposition 
\begin{align*}
    A = P \begin{bmatrix} 
    \lambda_1 & &  \\
     & \ddots &  \\
     &  & \lambda_n 
    \end{bmatrix} P^\dagger.
\end{align*}
Assume that the eigenvalues of $A$ are contained in a real interval $[a,b]$.
For a function $f: [a,b] \to \R$, we define a Hermitian matrix $f(A) \in \C^{n\times n}$ as
\begin{align*}
    f(A) = P \begin{bmatrix} 
    f(\lambda_1) & &  \\
     & \ddots &  \\
     &  & f(\lambda_n)
    \end{bmatrix} P^\dagger.
\end{align*}
Especially, for a positive semidefinite $A$ and $f(x) = x^{1/2}$, we write $A^{1/2} = f(A)$.
Similarly, we define $\exp(A)$ for a Hermitian $A$ and $\log(A)$ for a positive definite $A$.


For positive definite matrices $A$ and $B$, its \emph{geometric mean} $A\# B$ is defined as 
\begin{align*}
    A \# B = A^{1/2}(A^{-1/2}B A^{-1/2})^{1/2} A^{1/2}.
\end{align*}
It is well known that $A \# B$ is positive definite and $A\# B = B \# A$.
Furtheremore, $A\# B$ is the unique positive definite solution of a \emph{Riccati equation} $XBX = A$.

A \emph{(continous time) Lyapunov equation} is the following matrix equation 
\begin{align*}
    A^\dagger X + X A = Q,
\end{align*}
where $A$ and $Q$ are given marices.
It is well-known that if $A$ is positively stable (i.e., all the eigenvalues of $A$ are contained in the open right half-plane of $\C$), then the Lyapunov equation has the unique solution
\begin{align*}
    X = \int_{0}^{\infty} e^{-tA^\dagger} Q e^{tA} dt.
\end{align*}
Furtheremore, if $A$ and $Q$ are Hermitian matrices, then the solution is also Hermitian.
